Curvature-driven pathways interpolating between stationary points: the case of the pure spherical 3-spin model

This paper focuses on characterizing the energy profile along pathways connecting different regions of configuration space in the context of a prototypical glass model, the pure spherical $p$-spin model with $p=3$. The study investigates pairs of stationary points (local minima or rank-1 saddles), analyzing the energy profile along geodesic paths and comparing them with "perturbed" pathways correlated to the landscape curvature. The goal is to assess the extent to which information from the local Hessian matrices around stationary points can identify paths with lower energy barriers. Surprisingly, unlike findings in other systems, the direction of softest local curvature is not a reliable predictor of low-energy paths, except in the case in which the direction of softest curvature corresponds to an isolated mode of the Hessian. However, other information encoded in the local Hessian does allow the identification of pathways associated with lower energy barriers. We conclude commenting on implications for the system's activated dynamics.

==> settings_custom.tex <==
% Shorthands
\def\new{\text{new}}
\def\iid{\text{i.i.d.}}
\newcommand{\extr}{\textrm{\textbf{extr}}}
\newcommand{\argmin}{\textrm{argmin}}
\newcommand{\prox}{\textrm{prox}}
\newcommand{\tot}{\textrm{tot}}

% Integral measures
\def\dd{\text{d}}

% Special functions
\def\sign{\text{sign}}
\def\erf{\text{erf}}
\def\relu{\text{relu}}


% Fixme and todo commands
\newcommand{\fixme}[1]{{\sffamily\normalsize\bfseries \underline{FIXME:} } { \color{red} #1} \\}

\newcommand{\todo}[1]{{\sffamily\normalsize\bfseries {\underline{\color{blue}TODO:}} } { \color{blue} #1}}

% Define theorem environment
\newtheorem{theorem}{Theorem}

%%Operators
\DeclareMathOperator{\Prox}{Prox}
\DeclareMathOperator*{\Extr}{Extr}
\DeclareMathOperator*{\Argmin}{argmin}

%%%%% Bold font
\newcommand{\bsA}{{\boldsymbol{\mathsf A}}}
\newcommand{\bG}{{\boldsymbol{G}}}
\newcommand{\bT}{{\boldsymbol{T}}}
\newcommand{\bOne}{{\boldsymbol{1}}}
\newcommand{\bR}{{\boldsymbol{R}}}
\newcommand{\bhR}{{\hat{\boldsymbol{R}}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bH}{{\boldsymbol{H}}}
\newcommand{\bA}{{\boldsymbol{A}}}
\newcommand{\bC}{{\boldsymbol{C}}}
\newcommand{\bS}{{\boldsymbol{S}}}
\newcommand{\bhS}{{\hat{\boldsymbol{S}}}}
\newcommand{\bU}{{\boldsymbol{U}}}
\newcommand{\bhU}{{\hat{\boldsymbol{U}}}}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bW}{{{\boldsymbol{{W}}}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bQ}{{\boldsymbol{Q}}}
\newcommand{\bV}{{\boldsymbol{V}}}
\newcommand{\bsQ}{{\boldsymbol{\mathsf Q}}}
\newcommand{\bsS}{{\boldsymbol{\mathsf S}}}
\newcommand{\bM}{{\boldsymbol{m}}}
\newcommand{\bhQ}{{\hat{\boldsymbol{Q}}}}
\newcommand{\bhV}{{\hat{\boldsymbol{V}}}}
\newcommand{\bhM}{{\hat{\boldsymbol{m}}}}
\newcommand{\bMM}{{{\boldsymbol{M}}}}
\newcommand{\bhMM}{{\hat{\boldsymbol{M}}}}
\newcommand{\bbb}{{\boldsymbol{b}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bbB}{{\boldsymbol{B}}}
\newcommand{\bF}{{\boldsymbol{F}}}
\newcommand{\bZ}{{\boldsymbol{Z}}}
\newcommand{\bY}{{\boldsymbol{Y}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bPi}{{\boldsymbol{\Pi}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bsigma}{{\boldsymbol{\sigma}}}
\newcommand{\blambda}{{\boldsymbol{\lambda}}}
\newcommand{\bomega}{{\boldsymbol{\omega}}}
\newcommand{\bzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bXi}{{\boldsymbol{\Xi}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bI}{{\boldsymbol{I}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bff}{{\boldsymbol{f}}}
\newcommand{\be}{{\boldsymbol{e}}}
\newcommand{\beeta}{{\boldsymbol{\eta}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\bu}{{\boldsymbol{u}}}


% Matrix and vectors
\def\mat#1{\text{#1}}
\renewcommand{\vec}[1]{\bm{#1}}
